Active Electrosensing and Communication in MARL-trained Weakly Electric Fish Collectives

How complex collective behavior emerges from individual interactions is a fundamental scientific question, but experimental cost and difficulty of simultaneous multi-brain recordings limit direct study in animals. Here we introduce a novel computational framework modeling weakly electric fish-like agents with biophysically inspired electrosensing and actuation, trained to forage collectively via multi-agent reinforcement learning (MARL). Trained agents reproduce hallmarks of real fish, including curvilinear homing trajectories and heavy-tailed electric organ discharge (EOD) interval statistics, while exhibiting emergent active sensing, social foraging, dominance-like asymmetries, and aggression. We perform in silico interventions including sensor ablations, EOD silencing, and food distribution changes to identify causal drivers of social foraging. Analyses of recurrent neural dynamics further show robust encoding of task-relevant variables and social context. Our work has broad implications for the neuroethology of weakly electric fish and other social animals where extensive multi-individual neural recordings, and thus traditional data-driven modeling, remain challenging.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        # system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sensing_math_include.tex <==

\newpage
% \onecolumn % Redundant
\appendix
\section{Appendix: Basic Electrostatic Calculations}
\label{supp:calibration}
\subsection{Dipole Moment for a Given Maximum Field at Distance \( x \)}

The electric field ($\bm{E}$) of a dipole at a point $\bm{r}$ (where $x = |\bm{r}|$) is given by the general vector formula:
\[
\bm{E}(\bm{r}) = \frac{1}{4 \pi \varepsilon_0} \left[ \frac{3(\bm{p} \cdot \hat{\bm{r}})\hat{\bm{r}} - \bm{p}}{x^3} \right]
\]
where $\bm{p}$ is the dipole moment vector and $\hat{\bm{r}}$ is the unit vector in the direction of $\bm{r}$.
Alternatively, in spherical coordinates the magnitude of the electric field at a point ($x, \theta$) is:
\[
E(x, \theta) = \frac{p}{4 \pi \varepsilon_0 x^3} \sqrt{3\cos^2\theta + 1}
\]
where $\theta$ is the angle between the dipole moment vector $\bm{p}$ and the position vector $\bm{r}$.


The magnitude of the electric field ($E$) is maximized when $\cos\theta = \pm 1$, which corresponds to an angle of $\theta = 0^{\circ}$ or $\theta = 180^{\circ}$, i.e. directly along the axis of the dipole. 
The field magnitude along the axis is then:
\[
E_{\text{max}} = \frac{p}{2 \pi \varepsilon_0 x^3}
\]

Therefore, the dipole moment \( p \) required to generate a maximum electric field \( E_{\text{max}} \) at a distance \( x \) is:
\[
p = 2 \pi \varepsilon_0 x^3 E_{\text{max}}
\]
where $p$ is the dipole moment (C$\cdot$m), $x$ is the distance from the dipole where the field is maximized (m), $E_{\text{max}}$ is the required electric field magnitude (V/m), and $\varepsilon_0$ is the permittivity of free space ($8.854 \times 10^{-12}$ F/m).


\subsection{Dipole Moment Required to Induce a Specific Field at Its Own Location}

Active sensing involves three steps: a source dipole ($\bm{p}$) creates a field, this field induces a new dipole ($\bm{p}'$) on a conductor (other agent or prey), and this induced dipole in turn creates a field that the source's sensors detect.

To calibrate the strength of the EOD source, we find the source dipole moment ($p$) such that the maximum induced field at the source's location, $E_{\text{induced}}$, is equal to a desired value, $E_{\text{max}}$.

The electric field at the conductor due to the source dipole is given by the on-axis formula:
\[
E_{\text{source}} = \frac{p}{2 \pi \varepsilon_0 x^3}
\]

This source field induces a dipole moment ($\bm{p}'$) on the conductor, which is assumed to be a sphere of radius $R$:
\[
p' = 3 \varepsilon_0 V \cdot \chi \cdot E_{\text{source}}
\]
where $V = \frac{4}{3} \pi R^3$ is the volume of the conductor. 

Substituting the expression for $E_{\text{source}}$ and simplifying yields:
\[
p' = 3 \varepsilon_0 \left( \frac{4}{3} \pi R^3 \right) \cdot \chi \cdot \frac{p}{2 \pi \varepsilon_0 x^3} = \frac{2 R^3 \cdot \chi \cdot p}{x^3}
\]


The induced dipole ($\bm{p}'$) then creates its own on-axis electric field at the location of the original source dipole. The magnitude of this induced field is:
\[
E_{\text{induced}} = \frac{p'}{2 \pi \varepsilon_0 x^3}
\]
Substituting the simplified expression for $p'$ into this equation, we get:
\[
E_{\text{induced}} = \frac{1}{2 \pi \varepsilon_0 x^3} \left( \frac{2 R^3 \cdot \chi \cdot p}{x^3} \right) = \frac{R^3 \cdot \chi \cdot p}{\pi \varepsilon_0 x^6}
\]

To calibrate the source EOD dipole strength, we set this induced field equal to the sensor's minimum detection threshold, $E_{\text{max}}$ and solve for the required source dipole moment, $p$:
\[
p = \frac{E_{\text{max}} \pi \varepsilon_0 x^6}{R^3 \cdot \chi}
\]
where,
$p$ is the required dipole moment of the source (C$\cdot$m),
$E_{\text{max}}$ is the target electric field magnitude at the source dipole (V/m),
$x$ is the separation between the source dipole and the conductor (m),
$R$ is the conductor’s radius (m),
$\chi$ is the conductor contrast factor,
$\varepsilon_0$ is the permittivity of free space ($8.854 \times 10^{-12}$ F/m).


%%%%%%%%%%%%%%%%%
\newpage
\section{Appendix: Sensing range sanity checks}
\label{supp:range_checks}

\subsection{Self-EOD vs. Induced-dipole field strength at a Mormyromast sensor (on-axis, collinear)}

Consider a source dipole at $(0,0)$ with moment $\bm p=p\,\hat{\bm y}$, a spherical object of radius $R$ centered at $(0,x_{\text{obj}})$, and a Mormyromast-type sensor on the source body at $(0,r)$ with outward normal $\hat{\bm y}$. 
All positions are collinear along $\hat{\bm y}$ and fields are evaluated on-axis.

\paragraph{Self field at the sensor:}
On-axis self-EOD field magnitude at $(0,r)$:
\[
E_{\text{self}}=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{r^3}\right|.
\]

\paragraph{Induced field at the sensor:}
Field at the object’s center:
\[
E_{\text{source}\to\text{obj}}=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{x_{\text{obj}}^3}\right|.
\]
Assuming object is a sphere with contrast factor $\chi$ the induced dipole moment is
\[
p' \;=\; 4\pi\varepsilon_0 R^3\,\chi\,E_{\text{source}\to\text{obj}}
\;=\; \frac{2 R^3 \chi}{x_{\text{obj}}^3}\,p.
\]

The field magnitude at $(0,r)$ due to the induced dipole at $(0,x_{\text{obj}})$ is
\[
E_{\text{ind}}=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p'}{|x_{\text{obj}}-r|^3}\right|
=\frac{1}{2\pi\varepsilon_0}\,\frac{1}{|x_{\text{obj}}-r|^3}\left(\frac{2 R^3 \chi}{x_{\text{obj}}^3}p\right).
\]

\paragraph{Ratio (self vs.\ induced).}
Taking the ratio of magnitudes,
\[
\frac{E_{\text{self}}}{E_{\text{ind}}}
\;=\;
\frac{\displaystyle \frac{p}{2\pi\varepsilon_0 r^3}}
{\displaystyle \frac{1}{2\pi\varepsilon_0}\frac{2 R^3 \chi}{x_{\text{obj}}^3}\frac{p}{|x_{\text{obj}}-r|^3}}
\;=\;
\boxed{\;\frac{x_{\text{obj}}^{3}\,|x_{\text{obj}}-r|^{3}}{2\,\chi\,R^{3}\,r^{3}}\,.\;}
\]
In the common regime $r\ll x_{\text{obj}}$, $|x_{\text{obj}}-r|\approx x_{\text{obj}}$ and
\[
\frac{E_{\text{self}}}{E_{\text{ind}}}\;\approx\;\frac{x_{\text{obj}}^{6}}{2\,\chi\,R^{3}\,r^{3}}.
\]

\noindent For a prey object that is $x_{obj}=5$ cm away, with $R=0.25$ cm radius, \\ $|\chi| = 0.5$, and agent radius $r=1$ cm,
$\frac{E_{\text{self}}}{E_{\text{ind}}}\;\approx\; 10^6$
\\

\noindent For a post-baseline-subtraction sensing dynamic range of 10 (``one order of magnitude'') on $E_{ind}$, i.e.:
$E^B_{ind} / E^A_{ind} = 10$, implies a distance range of $x^A_{obj} / x^B_{obj} = 10^{1/6} = 1.47 = 1/(0.68)$



%%%%%%%%%%%%%%%%%
\newpage
\subsection{Self-EOD vs. Cons-EOD field strength at a Mormyromast sensor (on-axis, collinear)}

Given two agents, one at $(0,0)$ and the conspecific agent at $(0, x_{cons})$, we will calculate the ratio between the field due to self-EOD $E_{\text{self-EOD}}$ and due to cons-EOD $E_{\text{cons-EOD}}$ at a Mormyromast-type sensor located at $(0, r)$ with a radially-outward pointing normal. 

For simplicity, we assume that a point dipole $\bm p = p\,\hat{\bm y}$ at the first agent's center generates the \emph{self-EOD}. 
When a conspecific emits (receiver is not emitting), the
conspecific dipole (assumed collinear and aligned) at $y=x_{\text{cons}}>r$ on the $+\hat{\bm y}$
axis. 

The on-axis dipole field is given by
\[
E_y^{(\text{dip})}(\Delta y)=\frac{1}{2\pi\varepsilon_0}\;p\;\frac{\operatorname{sgn}(\Delta y)}{|\Delta y|^3},
\]
% and denote by $E_{\text{self-EOD}}$ the (known) magnitude of the self field at the sensor.

$E_{\text{self-EOD}}$, the magnitude of the self-EOD field at the sensor is given by:

\[
E_{\text{self-EOD}}
=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p_{\text{self}}}{r^3}\right|.
\]
% Hence
% \[
% \frac{p_{\text{self}}}{2\pi\varepsilon_0}=E_{\text{self-EOD}}\,r^3.
% \]

$E_{\text{cons-EOD}}$, the magnitude of the cons-EOD field, due to a dipole at $(0, x_{\text{cons}})$, at the same sensor is given by:
\[
E_{\text{cons-EOD}}
=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p_{\text{cons}}}{|x_{\text{cons}}-r|^3}\right|.
\]

Assuming same dipole strength, their ratio is given by
$$
\frac{ E_{\text{self-EOD}} }{ E_{\text{cons-EOD}} } = 
\frac{|x_{\text{cons}}-r|^3}{ r^3 }
$$

\noindent For agents separated by $ x_{cons} \approx 10$ cm and a agent body radius $r \approx 1$ cm, \\
$ E_{\text{self-EOD}} / E_{\text{cons-EOD}} = 9^3 = 729$.
% \\
% For $r=2$, $\frac{ E_{\text{self-EOD}} }{ E_{\text{cons-EOD}} } \approx ((10-2)/2)^3 = 64$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\subsection{Cons-EOD (direct) vs. Food-induced field at a Mormyromast sensor (on-axis, collinear)}

Consider a receiver at $(0,0)$ with a Mormyromast-type sensor located at $(0,r)$ and outward normal $\hat{\bm y}$. 
A conspecific is centered at $(0,x_{\text{cons}})$ and emits a dipole moment $\bm p = p\,\hat{\bm y}$. 
A spherical object (``food'') of radius $R$ and contrast factor $\chi$ is centered at $(0,x_{\text{food}})$ on the same axis. 
All fields are evaluated on-axis along $\hat{\bm y}$.

\paragraph{Direct conspecific field at the sensor.}
For an on-axis dipole, the $y$-component of the electric field at separation $\Delta y$ is
\[
E_y^{(\text{dip})}(\Delta y)\;=\;\frac{1}{2\pi\varepsilon_0}\;p\;\frac{\operatorname{sgn}(\Delta y)}{|\Delta y|^3}.
\]
Thus, the (magnitude of the) direct field from the conspecific at the sensor is
\[
E_{\text{cons}}
\;=\;
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{|x_{\text{cons}}-r|^3}\right|.
\]

\paragraph{Food-induced field at the sensor (driven by the conspecific).}
The conspecific’s field at the object location is
\[
E_{\text{cons}\to\text{obj}}
\;=\;
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{|x_{\text{food}}-x_{\text{cons}}|^3}\right|.
\]
Assuming a sphere with contrast $\chi$, the induced dipole at the object is
\[
p'
\;=\;
4\pi\varepsilon_0 R^3\,\chi\,E_{\text{cons}\to\text{obj}}
\;=\;
\frac{2\,R^3\,\chi}{|x_{\text{food}}-x_{\text{cons}}|^3}\;p.
\]
This induced dipole then produces, at the sensor position $(0,r)$, the on-axis field
\[
E_{\text{ind}}
\;=\;
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p'}{|x_{\text{food}}-r|^3}\right|
\;=\;
\frac{1}{2\pi\varepsilon_0}\;
\frac{1}{|x_{\text{food}}-r|^3}\;
\left(\frac{2\,R^3\,\chi}{|x_{\text{food}}-x_{\text{cons}}|^3}\,p\right).
\]

\paragraph{Ratio (induced vs.\ conspecific-direct).}
Taking the ratio of magnitudes,
\[
\frac{E_{\text{ind}}}{E_{\text{cons}}}
\;=\;
\frac{\displaystyle \frac{1}{2\pi\varepsilon_0}\frac{2 R^3 \chi}{|x_{\text{food}}-x_{\text{cons}}|^3}\frac{p}{|x_{\text{food}}-r|^3}}
{\displaystyle \frac{1}{2\pi\varepsilon_0}\frac{p}{|x_{\text{cons}}-r|^3}}
\;=\;
\boxed{\;
\frac{E_{\text{ind}}}{E_{\text{cons}}}
\;=\;
\frac{2\,|\chi|\,R^{3}\,|x_{\text{cons}}-r|^{3}}
{|x_{\text{food}}-x_{\text{cons}}|^{3}\,|x_{\text{food}}-r|^{3}}
\;}\!,
\]
where we have written $|\chi|$ to emphasize that the sign of $\chi$ only flips the induced field’s direction, while our interest here is in magnitudes.

\paragraph{Far-field scaling.}
In the common regime $r\ll x_{\text{food}}$ and $r\ll x_{\text{cons}}$, we have
$|x_{\text{food}}-r|\approx x_{\text{food}}$ and $|x_{\text{cons}}-r|\approx x_{\text{cons}}$, giving
\[
\frac{E_{\text{ind}}}{E_{\text{cons}}}
\;\approx\;
\frac{2\,|\chi|\,R^{3}\,x_{\text{cons}}^{3}}{x_{\text{food}}^{6}}.
\]
Hence, for fixed $x_{\text{cons}}$ the induced-to-cons ratio decays as $x_{\text{food}}^{-6}$: a one-decade increase in $E_{\text{ind}}$ corresponds to shrinking $x_{\text{food}}$ by a factor of $10^{1/6}\!\approx\!1.47$.

\paragraph{Numerical example.}
Let $R=0.25$ cm, $|\chi|=0.5$, $r=1$ cm, $x_{\text{cons}}=10$ cm, and $x_{\text{food}}=5$ cm. 
Using the far-field form,
\[
\frac{E_{\text{ind}}}{E_{\text{cons}}}
\;\approx\;
\frac{2(0.5)\,(0.25\,\text{cm})^{3}\,(10\,\text{cm})^{3}}{(5\,\text{cm})^{6}}
\;=\;
\frac{(0.25^{3})\cdot 10^{3}}{5^{6}}
\;\approx\;10^{-3}.
\]
Thus, at these distances the food-induced perturbation is about three orders of magnitude smaller than the direct conspecific field at the sensor.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ADD RECEIVER-INDUCED CHARGE 
\newpage
\subsection{Cons-EOD (direct) vs. Food-induced \emph{and} Receiver-induced fields (on-axis, collinear)}

We retain the same collinear geometry: the receiver is centered at $(0,0)$ with a Mormyromast sensor at $(0,r)$ (outward normal $\hat{\bm y}$), a conspecific is centered at $(0,x_{\text{cons}})$ and emits a dipole $\bm p=p\,\hat{\bm y}$, and a spherical ``food'' object of radius $R$ and contrast $\chi$ is centered at $(0,x_{\text{food}})$. 
We additionally assume the receiver body (radius $r$) has the \emph{same} contrast $\chi$ and can be polarized by external fields.

\paragraph{Direct conspecific field at the sensor.}
As before, the on-axis dipole field gives
\[
E_{\text{cons}}
=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{|x_{\text{cons}}-r|^3}\right|.
\]

\paragraph{Food-induced field at the sensor (driven by the conspecific).}
The conspecific produces at the food location
\[
E_{\text{cons}\to\text{food}}
=\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{|x_{\text{food}}-x_{\text{cons}}|^3}\right|,
\qquad
p'_{\text{food}}
=4\pi\varepsilon_0 R^3 \chi\,E_{\text{cons}\to\text{food}}
=\frac{2 R^3 \chi}{|x_{\text{food}}-x_{\text{cons}}|^3}\,p.
\]
The induced dipole at the food contributes at the sensor
\[
E_{\text{ind,food}}
=
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p'_{\text{food}}}{|x_{\text{food}}-r|^3}\right|
=\frac{1}{2\pi\varepsilon_0}\,
\frac{2\,|\chi|\,R^3}{|x_{\text{food}}-x_{\text{cons}}|^3\,|x_{\text{food}}-r|^3}\,p.
\]

\paragraph{Receiver-induced field at the sensor (polarization of the non-emitter).}
The conspecific’s field at the \emph{receiver} center is
\[
E_{\text{cons}\to\text{recv}}
=
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p}{|x_{\text{cons}}|^3}\right|.
\]
Treating the receiver as a polarizable sphere (radius $r$, contrast $\chi$), the induced dipole at the receiver is
\[
p'_{\text{recv}}
=4\pi\varepsilon_0 r^3 \chi\,E_{\text{cons}\to\text{recv}}
=\frac{2 r^3 \chi}{|x_{\text{cons}}|^3}\,p,
\]
which produces at the surface sensor $(0,r)$ the on-axis dipole field
\[
E_{\text{ind,recv}}
=
\left|\frac{1}{2\pi\varepsilon_0}\,\frac{p'_{\text{recv}}}{r^3}\right|
=\frac{1}{2\pi\varepsilon_0}\,\frac{2\,|\chi|}{|x_{\text{cons}}|^3}\,p.
\]
(Note the cancellation of $r^3$; the magnitude at the surface is independent of $r$ in this ideal spherical model.)

\paragraph{Total sensed field (no baseline subtraction).}
\[
E_{\text{tot}}
\;=\;
E_{\text{cons}}+E_{\text{ind,food}}+E_{\text{ind,recv}}.
\]

\paragraph{Ratios with respect to the direct conspecific field.}
Dividing each contribution by $E_{\text{cons}}$ yields
\[
\frac{E_{\text{ind,food}}}{E_{\text{cons}}}
=
\frac{2\,|\chi|\,R^{3}\,|x_{\text{cons}}-r|^{3}}
{|x_{\text{food}}-x_{\text{cons}}|^{3}\,|x_{\text{food}}-r|^{3}},
\qquad
\frac{E_{\text{ind,recv}}}{E_{\text{cons}}}
=
\frac{\displaystyle \frac{2\,|\chi|}{|x_{\text{cons}}|^{3}}}
{\displaystyle \frac{1}{|x_{\text{cons}}-r|^{3}}}
=
2\,|\chi|\,\frac{|x_{\text{cons}}-r|^{3}}{|x_{\text{cons}}|^{3}}.
\]
Hence the combined induced-to-cons ratio is
\[
\boxed{~
\frac{E_{\text{ind,food}}+E_{\text{ind,recv}}}{E_{\text{cons}}}
\;=\;
2\,|\chi|\;|x_{\text{cons}}-r|^{3}
\left[
\frac{R^{3}}{|x_{\text{food}}-x_{\text{cons}}|^{3}\,|x_{\text{food}}-r|^{3}}
\;+\;
\frac{1}{|x_{\text{cons}}|^{3}}
\right].
~}
\]


==> supp_features_table.tex <==
\subsection{List of recurrent-state decoding targets}
\begin{table}[ht]
\centering
\small
\begin{tabular}{llll}
\toprule
\textbf{Target} & \textbf{Code field} & \textbf{Type} & \textbf{Description} \\
\midrule
Position X & \texttt{position\_x} & Scalar & Allocentric x position \\
Position Y & \texttt{position\_y} & Scalar & Allocentric y position \\
Distance to Nearest Agent & \texttt{distance\_to\_nearest\_agent} & Scalar & Distance to closest conspecific \\
Distance to Closest Food & \texttt{distance\_to\_closest\_food} & Scalar & Distance to nearest food item \\
Angle to Closest Agent & \texttt{angle\_to\_closest\_agent} & Circular & Bearing to closest conspecific \\
Angle to Closest Food & \texttt{angle\_to\_closest\_food} & Circular & Bearing to nearest food item \\
Actual Turn & \texttt{actual\_turn} & Scalar & Realized angular change per timestep \\
Agent Size & \texttt{agent\_size} & Scalar & Scalar size context of the focal agent \\
Energy & \texttt{energy} & Scalar & Internal energy state, when present in the rollout table \\
Agents in Knollen Range & \texttt{num\_agents\_in\_knollen\_range} & Count & Number of conspecifics within Knollenorgan range \\
Size of Nearest Agent & \texttt{size\_of\_nearest\_agent} & Scalar & Size metadata for the nearest conspecific \\
Distance to Second Nearest Agent & \texttt{distance\_to\_second\_nearest\_agent} & Scalar & Distance to the second-nearest conspecific \\
Size of Second Nearest Agent & \texttt{size\_of\_second\_nearest\_agent} & Scalar & Size metadata for the second-nearest conspecific \\
Food Count Centered & \texttt{food\_count\_5cm} & Count & Number of food items within the centered 5 cm local window \\
Food Count Front & \texttt{food\_front\_5cm} & Count & Number of food items in the 5 cm front sector \\
Food Count Behind & \texttt{food\_back\_5cm} & Count & Number of food items in the 5 cm rear sector \\
Food Count Left & \texttt{food\_left\_5cm} & Count & Number of food items in the 5 cm left sector \\
Food Count Right & \texttt{food\_right\_5cm} & Count & Number of food items in the 5 cm right sector \\
Agent Nearby & \texttt{has\_nearby} & Boolean & Whether a conspecific is within the nearby-agent threshold \\
Was Bitten & \texttt{was\_bitten} & Boolean & Whether the agent was bitten on that timestep \\
Agent in Knollen Range & \texttt{has\_agent\_in\_knollen\_range} & Boolean & Whether any conspecific is within Knollenorgan range \\
Knollen Error Angle & \texttt{knollen\_error\_angle} & Circular & Derived orientation error relative to the Knollenorgan field direction \\
Mormyromast Field Magnitude & \texttt{mormyromast\_field\_mag\_log} & Scalar & Log-transformed Mormyromast field magnitude, when available \\
Ampullary Field Magnitude & \texttt{ampullary\_field\_mag\_log} & Scalar & Log-transformed Ampullary field magnitude, when available \\
Mormyromast Error Angle & \texttt{mormyromast\_error\_angle} & Circular & Homing-task error angle for the Mormyromast field \\
Ampullary Error Angle & \texttt{ampullary\_error\_angle} & Circular & Homing-task error angle for the Ampullary field \\
Knollen Error Angle to Nearest Agent & \texttt{knollen\_error\_angle\_nearest} & Circular & Homing-task error angle for the nearest-agent Knollen field \\
\bottomrule
\end{tabular}
\caption{Current recurrent-state decoding targets. The decoder builds this list from rollout columns, derived field features, and the exclusion list in \texttt{features.py}; targets absent from a given assay are skipped. Archived action-prediction targets, including binned movement commands and future EOD-probability classes, are not part of the current manuscript pipeline.}
\label{tab:features}
\end{table}

